A Perception-Based L2 Speech Intelligibility Indicator: Leveraging a Rater's Shadowing and Sequence-to-sequence Voice Conversion

Evaluating L2 speech intelligibility is crucial for effective computer-assisted language learning (CALL). Conventional ASR-based methods often focus on native-likeness, which may fail to capture the actual intelligibility perceived by human listeners. In contrast, our work introduces a novel, perception based L2 speech intelligibility indicator that leverages a native rater's shadowing data within a sequence-to-sequence (seq2seq) voice conversion framework. By integrating an alignment mechanism and acoustic feature reconstruction, our approach simulates the auditory perception of native listeners, identifying segments in L2 speech that are likely to cause comprehension difficulties. Both objective and subjective evaluations indicate that our method aligns more closely with native judgments than traditional ASR-based metrics, offering a promising new direction for CALL systems in a global, multilingual contexts.

==> mybib.tex <==
@inproceedings{zhao2018l2arctic,
    author={Guanlong {Zhao} and Sinem {Sonsaat} and Alif {Silpachai} and Ivana {Lucic} and Evgeny {Chukharev-Hudilainen} and John {Levis} and Ricardo {Gutierrez-Osuna}},
    title={L2-ARCTIC: A Non-native English Speech Corpus},
    year=2018,
    booktitle={Proc. Interspeech},
    pages={2783–2787},
}
@online{wang2024globe,
title={GLOBE: A High-quality English Corpus with Global Accents for Zero-shot Speaker Adaptive Text-to-Speech}, 
author={Wenbin Wang and Yang Song and Sanjay Jha},
year={2024},
eprint={2406.14875},
}

@inproceedings{geng2024APSIPA,
  author       = {Haopeng Geng and
                  Daisuke Saito and
                  Nobuaki Minematsu and
                  },
  title        = {A Pilot Study of Applying Sequence-to-Sequence Voice Conversion to Evaluate the Intelligibility of L2 Speech Using a Native Speaker’s Shadowings},
  booktitle    = {Proc. APSIPA ASC (submitted)} ,
  year         = {2024},
}

@ARTICLE{yangspeechfound,
  author={Yang, Shu-wen and Chang, Heng-Jui and Huang, Zili and Liu, Andy T. and Lai, Cheng-I and Wu, Haibin and Shi, Jiatong and Chang, Xuankai and Tsai, Hsiang-Sheng and Huang, Wen-Chin and Feng, Tzu-hsun and Chi, Po-Han and Lin, Yist Y. and Chuang, Yung-Sung and Huang, Tzu-Hsien and Tseng, Wei-Cheng and Lakhotia, Kushal and Li, Shang-Wen and Mohamed, Abdelrahman and Watanabe, Shinji and Lee, Hung-yi},
  journal={IEEE/ACM TASLP}, 
  title={A Large-Scale Evaluation of Speech Foundation Models}, 
  year={2024},
  volume={32},
  number={},
  pages={2884-2899}
}


@article{saeki2022utmos,
  title={UTMOS: UTokyo-SaruLab System for VoiceMOS Challenge 2022},
  author={Saeki, Takaaki and Xin, Detai and Nakata, Wataru and Koriyama, Tomoki and Takamichi, Shinnosuke and Saruwatari, Hiroshi},
  journal={Proc. Interspeech},
  year={2022},
  pages={4521--4525},
}
@inproceedings{DBLP:conf/iclr/ZhangKWWA20,
  author       = {Tianyi Zhang and
                  Varsha Kishore and
                  Felix Wu and
                  Kilian Q. Weinberger and
                  Yoav Artzi},
  title        = {BERTScore: Evaluating Text Generation with {BERT}},
  booktitle    = {ICLR} ,
  year         = {2020},
}
@inproceedings{tomita24_interspeech,
  title     = {Analysis and Visualization of Directional Diversity in Listening Fluency of World Englishes Speakers in the Framework of Mutual Shadowing},
  author    = {Yu Tomita and Yingxiang Gao and Nobuaki Minematsu and Noriko Nakanishi and Daisuke Saito},
  year      = {2024},
  booktitle = {Proc. Interspeech},
  pages     = {4024--4028},
}
@article{kong2020hifi,
  title={Hifi-gan: Generative adversarial networks for efficient and high fidelity speech synthesis},
  author={Kong, Jungil and Kim, Jaehyeon and Bae, Jaekyoung},
  journal={Proc. NeurIPS},
  volume={33},
  pages={17022--17033},
  year={2020}
}
@article{zhang2019non,
  title={Non-parallel sequence-to-sequence voice conversion with disentangled linguistic and speaker representations},
  author={Zhang, Jing-Xuan and Ling, Zhen-Hua and Dai, Li-Rong},
  journal={IEEE/ACM TASLP},
  volume={28},
  pages={540--552},
  year={2019},
}
@inproceedings{violeta2024electrolaryngeal,
  title={Electrolaryngeal Speech Intelligibility Enhancement through Robust Linguistic Encoders},
  author={Violeta, Lester Phillip and Huang, Wen-Chin and Ma, Ding and Yamamoto, Ryuichi and Kobayashi, Kazuhiro and Toda, Tomoki},
  booktitle={Proc. ICASSP},
  year={2024},
  pages={10961--10965},
}
@inproceedings{wang2024unit,
  title={UNIT-DSR: Dysarthric Speech Reconstruction System Using Speech Unit Normalization},
  author={Wang, Yuejiao and Wu, Xixin and Wang, Disong and Meng, Lingwei and Meng, Helen},
  booktitle={Proc. ICASSP},
  pages={12306--12310},
  year={2024},
}

@article{saeki2024spbertscore,
  title={{SpeechBERTScore}: Reference-Aware Automatic Evaluation of Speech Generation Leveraging NLP Evaluation Metrics},
  author={Takaaki Saeki and Soumi Maiti and Shinnosuke Takamichi and Shinji Watanabe and Hiroshi Saruwatari},
  journal={arXiv preprint arXiv:2401.16812},
  year={2024}
}
@article{zhang2019bertscore,
  title={Bertscore: Evaluating text generation with bert},
  author={Zhang, Tianyi and Kishore, Varsha and Wu, Felix and Weinberger, Kilian Q and Artzi, Yoav},
  journal={arXiv preprint arXiv:1904.09675},
  year={2019}
}

@inproceedings{qian2022contentvec,
  title={Contentvec: An improved self-supervised speech representation by disentangling speakers},
  author={Qian, Kaizhi and Zhang, Yang and Gao, Heting and Ni, Junrui and Lai, Cheng-I and Cox, David and Hasegawa-Johnson, Mark and Chang, Shiyu},
  booktitle={Proc. ICML},
  pages={18003--18017},
  year={2022},
  organization={PMLR}
}

@article{ma2023can,
  title={Can generative large language models perform asr error correction?},
  author={Ma, Rao and Qian, Mengjie and Manakul, Potsawee and Gales, Mark and Knill, Kate},
  journal={arXiv preprint arXiv:2307.04172},
  year={2023}
}

@inproceedings{weng2020joint,
  title={Joint contextual modeling for asr correction and language understanding},
  author={Weng, Yue and Miryala, Sai Sumanth and Khatri, Chandra and Wang, Runze and Zheng, Huaixiu and Molino, Piero and Namazifar, Mahdi and Papangelis, Alexandros and Williams, Hugh and Bell, Franziska and others},
  booktitle={Proc. ICASSP},
  pages={6349--6353},
  year={2020},
}

@article{munro1995foreign,
  title={Foreign accent, comprehensibility, and intelligibility in the speech of second language learners},
  author={Munro, Murray J and Derwing, Tracey M},
  journal={Language learning},
  volume={45},
  number={1},
  pages={73--97},
  year={1995},
}

@article{Derwing_Munro_1997, title={ACCENT, INTELLIGIBILITY, AND COMPREHENSIBILITY: Evidence from Four L1s}, volume={19}, number={1}, journal={Studies in Second Language Acquisition}, author={Derwing, Tracey M. and Munro, Murray J.}, year={1997}, pages={1–16}} <div></div>

@article{hsu2021hubert,
  title={Hubert: Self-supervised speech representation learning by masked prediction of hidden units},
  author={Hsu, Wei-Ning and Bolte, Benjamin and Tsai, Yao-Hung Hubert and Lakhotia, Kushal and Salakhutdinov, Ruslan and Mohamed, Abdelrahman},
  journal={IEEE/ACM TASLP},
  volume={29},
  pages={3451--3460},
  year={2021},
}

@article{chen2022wavlm,
  title={Wavlm: Large-scale self-supervised pre-training for full stack speech processing},
  author={Chen, Sanyuan and Wang, Chengyi and Chen, Zhengyang and Wu, Yu and Liu, Shujie and Chen, Zhuo and Li, Jinyu and Kanda, Naoyuki and Yoshioka, Takuya and Xiao, Xiong and others},
  journal={IEEE JSTSP},
  volume={16},
  number={6},
  pages={1505--1518},
  year={2022},
}

@ARTICLE{lester_EL,
  author={Violeta, Lester Phillip and Ma, Ding and Huang, Wen-Chin and Toda, Tomoki},
  journal={IEEE/ACM TASLP}, 
  title={Pretraining and Adaptation Techniques for Electrolaryngeal Speech Recognition}, 
  year={2024},
  volume={32},
  number={},
  pages={2777-2789},
  keywords={Speech recognition;Task analysis;Pathology;Training;Neural networks;Transfer learning;Linguistics;Automatic speech recognition (ASR);domain adaptation;electrolaryngeal (EL) speech;model pretraining;low-resourced ASR},
}


@inproceedings{okamoto2023e2e,
  title={E2E-S2S-VC: End-to-end sequence-to-sequence voice conversion},
  author={Okamoto, Takuma and Toda, Tomoki and Kawai, Hisashi},
  booktitle={Proc. Interspeech},
  pages={2043--2047},
  year={2023}
}


@inproceedings{wav2vec2,
author = {Baevski, Alexei and Zhou, Henry and Mohamed, Abdelrahman and Auli, Michael},
title = {wav2vec 2.0: a framework for self-supervised learning of speech representations},
year = {2020},
booktitle = {Proc. NeurIPS},
articleno = {1044},
numpages = {12},
}

@inproceedings{maimon-adi-2023-speaking,
    title = "Speaking Style Conversion in the Waveform Domain Using Discrete Self-Supervised Units",
    author = "Maimon, Gallil  and Adi, Yossi",
    editor = "Bouamor, Houda  and Pino, Juan  and Bali, Kalika",
    booktitle = "EMNLP",
    year = "2023",
    pages = "8048--8061",
}
@INPROCEEDINGS{zhou_emotionVC,
  author={Zhou, Kun and Sisman, Berrak and Liu, Rui and Li, Haizhou},
  booktitle={Proc. ICASSP}, 
  title={Seen and Unseen Emotional Style Transfer for Voice Conversion with A New Emotional Speech Dataset}, 
  year={2021},
  volume={},
  number={},
  pages={920-924},
  keywords={Training;Emotion recognition;Speech recognition;Transforms;Signal processing;Linguistics;Electrostatic discharges;emotional voice conversion;speech emotion recognition (SER);emotional speech dataset},
}

@ARTICLE{zhao_fac_journal,
  author={Zhao, Guanlong and Ding, Shaojin and Gutierrez-Osuna, Ricardo},
  journal={IEEE/ACM TASLP}, 
  title={Converting Foreign Accent Speech Without a Reference}, 
  year={2021},
  volume={29},
  number={},
  pages={2367-2381},
  keywords={Synthesizers;Training;Acoustics;Speech processing;Decoding;Computational modeling;Transforms;Accent conversion;acoustic model;sequence-to-sequence voice conversion;speech modification;speech synthesis},
}

@inproceedings{chan22b_interspeech,
  author={May Pik Yu Chan and June Choe and Aini Li and Yiran Chen and Xin Gao and Nicole Holliday},
  title={{Training and typological bias in ASR performance for world Englishes}},
  year=2022,
  booktitle={Proc. Interspeech},
  pages={1273--1277},
  issn={2958-1796}
}
@inproceedings{lin2020shadowability,
  title={Shadowability Annotation with Fine Granularity on L2 Utterances and its Improvement with Native Listeners' Script-Shadowing.},
  author={Lin, Zhenchao and Takashima, Ryo and Saito, Daisuke and Minematsu, Nobuaki and Nakanishi, Noriko},
  booktitle={Proc. Interspeech},
  pages={3865--3869},
  year={2020}
}

@inproceedings{inoue18_interspeech,
  author={Yusuke Inoue and Suguru Kabashima and Daisuke Saito and Nobuaki Minematsu and Kumi Kanamura and Yutaka Yamauchi},
  title={{A Study of Objective Measurement of Comprehensibility through Native Speakers' Shadowing of Learners' Utterances}},
  year=2018,
  booktitle={Proc. Interspeech},
  pages={1651--1655}
}

@inproceedings{mine22_SP,
  author={Nobuaki Minematsu and Chuanbo Zhu and GiaBao Dangtran and
          Daisuke Saito and Nobiko Nakanishi and Kumi Kanamura},
  title={{Development of shadowing speech corpora to measure instantaneous intelligibility
          as sequential annotation on L2 speech}},
  year=2022,
  booktitle={Tech. Rep. Speech, Acoust. Soc. Jpn},
  pages={7--12}
}


@article{ren2020fastspeech,
  title={Fastspeech 2: Fast and high-quality end-to-end text to speech},
  author={Ren, Yi and Hu, Chenxu and Tan, Xu and Qin, Tao and Zhao, Sheng and Zhao, Zhou and Liu, Tie-Yan},
  journal={arXiv preprint arXiv:2006.04558},
  year={2020}
}
@inproceedings{hayashi2021non,
  title={Non-autoregressive sequence-to-sequence voice conversion},
  author={Hayashi, Tomoki and Huang, Wen-Chin and Kobayashi, Kazuhiro and Toda, Tomoki},
  booktitle={Proc. ICASSP},
  pages={7068--7072},
  year={2021},
}

@inproceedings{rasipuram2015automatic,
  title={Automatic accentedness evaluation of non-native speech using phonetic and sub-phonetic posterior probabilities},
  author={Rasipuram, Ramya and Cernak, Milos and Nanchen, Alexandre and others},
  booktitle={Proc. Interspeech},
  pages={648--652},
  year={2015}
}

@article{munro2020foreign,
  title={Foreign accent, comprehensibility and intelligibility, redux},
  author={Munro, Murray J and Derwing, Tracey M},
  journal={Journal of Second Language Pronunciation},
  volume={6},
  number={3},
  pages={283--309},
  year={2020},
}

@inproceedings{attention,
author = {Vaswani, Ashish and Shazeer, Noam and Parmar, Niki and Uszkoreit, Jakob and Jones, Llion and Gomez, Aidan N. and Kaiser, \L{}ukasz and Polosukhin, Illia},
title = {Attention is all you need},
year = {2017},
booktitle = {Proc. NeurIPS},
pages = {6000–6010},
numpages = {11},
}
@article{hamada2014effectiveness,
  title={The effectiveness of pre-and post-shadowing in improving listening comprehension skills},
  author={Hamada, Yo},
  journal={The Language Teacher},
  volume={38},
  number={1},
  pages={3--10},
  year={2014}
}
@article{neri2001effective,
  title={Effective feedback on L2 pronunciation in ASR-based CALL},
  author={Neri, Ambra and Cucchiarini, Catia and Strik, Helmer},
  year={2001},
}
@INPROCEEDINGS{9428161,
  author={Liu, Songxiang and Cao, Yuewen and Hu, Na and Su, Dan and Meng, Helen},
  booktitle={Proc. ICME}, 
  title={Fastsvc: Fast Cross-Domain Singing Voice Conversion With Feature-Wise Linear Modulation}, 
  year={2021},
  volume={},
  number={},
  pages={1-6},
  keywords={Multimedia systems;Conferences;Static VAr compensators;Modulation;Linguistics;Feature extraction;Signal generators;Singing voice conversion;cross-domain;generative adversarial network},
}

@inproceedings{yue17_interspeech,
  author={Junwei Yue and Fumiya Shiozawa and Shohei Toyama and Yutaka Yamauchi and Kayoko Ito and Daisuke Saito and Nobuaki Minematsu},
  title={{Automatic Scoring of Shadowing Speech Based on DNN Posteriors and Their DTW}},
  year=2017,
  booktitle={Proc. Interspeech},
  pages={1422--1426},
  issn={2958-1796}
}

@INPROCEEDINGS{9041215,
  author={Ando, Shintaro and Lin, Zhenchao and Trisitichoke, Tasavat and Inoue, Yusuke and Yoshizawa, Fuki and Saito, Daisuke and Minematsu, Nobuaki},
  booktitle={2019 22nd Conference of the Oriental COCOSDA International Committee for the Co-ordination and Standardisation of Speech Databases and Assessment Techniques (O-COCOSDA)}, 
  title={A Large Collection of Sentences Read Aloud by Vietnamese Learners of Japanese and Native Speaker's Reverse Shadowings}, 
  year={2019},
  volume={},
  number={},
  pages={1-6},
  keywords={second language learning;foreign accent;shadowing;comprehensibility;shadowability;GOP;DTW},
}

@inproceedings{
shih2021radtts,
title={RAD-TTS: Parallel Flow-Based {TTS} with Robust Alignment Learning and Diverse Synthesis},
author={Kevin J. Shih and Rafael Valle and Rohan Badlani and Adrian Lancucki and Wei Ping and Bryan Catanzaro},
booktitle={Proc. ICML},
year={2021},
}

@article{huang2023aas,
  title={AAS-VC: On the Generalization Ability of Automatic Alignment Search based Non-autoregressive Sequence-to-sequence Voice Conversion},
  author={Huang, Wen-Chin and Kobayashi, Kazuhiro and Toda, Tomoki},
  journal={arXiv preprint arXiv:2309.07598},
  year={2023}
}

@inproceedings{huang2021s3prl,
  title={S3PRL-VC: Open-source Voice Conversion Framework with Self-supervised Speech Representations},
  author={Huang, Wen-Chin and Yang, Shu-Wen and Hayashi, Tomoki and Lee, Hung-Yi and Watanabe, Shinji and Toda, Tomoki},
  booktitle={Proc. ICASSP},
  year={2022}
}
@ARTICLE{s3prl-vc-journal,
  author={Huang, Wen-Chin and Yang, Shu-Wen and Hayashi, Tomoki and Toda, Tomoki},
  journal={IEEE Journal of Selected Topics in Signal Processing}, 
  title={{A Comparative Study of Self-Supervised Speech Representation Based Voice Conversion}}, 
  year={2022},
  volume={16},
  number={6},
  pages={1308-1318},
}
@INPROCEEDINGS{6855134,
  author={Aryal, Sandesh and Gutierrez-Osuna, Ricardo},
  booktitle={Proc. ICASSP}, 
  title={Can voice conversion be used to reduce non-native accents?}, 
  year={2014},
  volume={},
  number={},
  pages={7879-7883},
  keywords={Vectors;Acoustics;Speech;Mathematical model;Transforms;Training;Pragmatics;Voice conversion;accent conversion;nonnative speech;Spanish accent},
}

@INPROCEEDINGS{zhao_ppg,
  author={Zhao, Guanlong and Sonsaat, Sinem and Levis, John and Chukharev-Hudilainen, Evgeny and Gutierrez-Osuna, Ricardo},
  booktitle={Proc. ICASSP}, 
  title={Accent Conversion Using Phonetic Posteriorgrams}, 
  year={2018},
  volume={},
  number={},
  pages={5314-5318},
  keywords={Acoustics;Phonetics;Computational modeling;Speech recognition;Transforms;Training;Testing;speech synthesis;accent conversion;frame pairing;posteriorgram;acoustic model},
}

@inproceedings{yamamoto2020parallel,
  title={Parallel WaveGAN: A fast waveform generation model based on generative adversarial networks with multi-resolution spectrogram},
  author={Yamamoto, Ryuichi and Song, Eunwoo and Kim, Jae-Min},
  booktitle={Proc. ICASSP},
  pages={6199--6203},
  year={2020},
}

@InProceedings{wills_et_al:OASIcs.SLATE.2023.7,
  author =	{Wills, Simone and Bai, Yu and Tejedor-Garc{\'\i}a, Cristian and Cucchiarini, Catia and Strik, Helmer},
  title =	{{Automatic Speech Recognition of Non-Native Child Speech for Language Learning Applications}},
  booktitle =	{Proc. SLATE},
  pages =	{7:1--7:8},
  year =	{2023},
}

@ARTICLE{liu2021any,
  author={Liu, Songxiang and Cao, Yuewen and Wang, Disong and Wu, Xixin and Liu, Xunying and Meng, Helen},
  journal={IEEE/ACM TASLP}, 
  title={Any-to-Many Voice Conversion With Location-Relative Sequence-to-Sequence Modeling}, 
  year={2021},
  volume={29},
  number={},
  pages={1717-1728},
}

@inproceedings{Liu2018,
  author={Songxiang Liu and Jinghua Zhong and Lifa Sun and Xixin Wu and Xunying Liu and Helen Meng},
  title={Voice Conversion Across Arbitrary Speakers Based on a Single Target-Speaker Utterance},
  year=2018,
  booktitle={Proc. Interspeech},
  pages={496--500},
}


@inproceedings{radford2023robust,
  title={Robust speech recognition via large-scale weak supervision},
  author={Radford, Alec and Kim, Jong Wook and Xu, Tao and Brockman, Greg and McLeavey, Christine and Sutskever, Ilya},
  booktitle={Proc. ICML},
  pages={28492--28518},
  year={2023},
}

@inproceedings{zhu2021multi,
  title={Multi-Granularity Annotation of Instantaneous Intelligibility of Learners' Utterances Based on Shadowing Techniques},
  author={Zhu, Chuanbo and Hakoda, Ryo and Saito, Daisuke and Minematsu, Nobuaki and Nakanishi, Noriko and Nishimura, Tazuko},
  booktitle={Proc. ASRU},
  pages={1071--1078},
  year={2021},
}

@INPROCEEDINGS{fac-evaluate,
  author={Wen-Chin Huang and Tomoki Toda},
  booktitle={Proc. APSIPA ASC},
  title={{Evaluating Methods for Ground-Truth-Free Foreign Accent Conversion}},
  year={2023},
}
@inproceedings{huang20i_interspeech,
  author={Wen-Chin Huang and Tomoki Hayashi and Yi-Chiao Wu and Hirokazu Kameoka and Tomoki Toda},
  title={{Voice Transformer Network: Sequence-to-Sequence Voice Conversion Using Transformer with Text-to-Speech Pretraining}},
  year=2020,
  booktitle={Proc. Interspeech},
  pages={4676--4680},
}
@ARTICLE{vtn_journal,
  author={Huang, Wen-Chin and Hayashi, Tomoki and Wu, Yi-Chiao and Kameoka, Hirokazu and Toda, Tomoki},
  journal={IEEE/ACM TASLP}, 
  title={Pretraining Techniques for Sequence-to-Sequence Voice Conversion}, 
  year={2021},
  volume={29},
  pages={745-755},
}


@article{Davis80-COP,
	Author = {Steven B. Davis and Paul Mermelstein},
	Journal = {IEEE TASLP},
	Number = {4},
	Pages = {357--366},
	Title = {Comparison of Parametric Representations for Monosyllabic Word Recognition in Continuously Spoken Sentences},
	Volume = {28},
  Month = aug,
	Year = {1980}}

@article{Rabiner89-ATO,
	Author = {Lawrence R. Rabiner},
	Journal = {Proceedings of the IEEE},
	Number = {2},
	Pages = {257--286},
	Title = {A Tutorial on Hidden {Markov} Models and Selected Applications in Speech Recognition},
	Volume = {77},
  Month = feb,
	Year = {1989}}

@inproceedings{shih2021rad,
  title={RAD-TTS: Parallel flow-based TTS with robust alignment learning and diverse synthesis},
  author={Shih, Kevin J and Valle, Rafael and Badlani, Rohan and Lancucki, Adrian and Ping, Wei and Catanzaro, Bryan},
  booktitle={ICML Workshop on Invertible Neural Networks, Normalizing Flows, and Explicit Likelihood Models},
  year={2021}
}
